Accelerated RRT* By Local Directional Visibility

RRT* is an efficient sampling-based motion planning algorithm. However, without taking advantages of accessible environment information, sampling-based algorithms usually result in sampling failures, generate useless nodes, and/or fail in exploring narrow passages. For this paper, in order to better utilize environment information and further improve searching efficiency, we proposed a novel approach to improve RRT* by 1) quantifying local knowledge of the obstacle configurations during neighbour rewiring in terms of directional visibility, 2) collecting environment information during searching, and 3) changing the sampling strategy biasing toward near-obstacle nodes after the first solution found. The proposed algorithm RRT* by Local Directional Visibility (RRT*-LDV) better utilizes local known information and innovates a weighted sampling strategy. The accelerated RRT*-LDV outperforms RRT* in convergence rate and success rate of finding narrow passages. A high Degree-Of-Freedom scenario is also experimented.

==> references.tex <==
abv

@article{RRT*,
  author = {S. Karaman and E. Frazzoli} , 
  title = {Sampling-based algorithms for optimal motion planning}, 
  volume = {30.}, 
  number = {7}, 
  pages = {846-894}, 
  year = {2011}, 
  journal = {International Journal of Robotics Research}
}

@article{SL,
  author = {Zhang X., Lütteke F., Ziegler C., Franke J.} , 
  title = {Self-learning RRT* Algorithm for Mobile Robot Motion Planning in Complex Environments}, 
  volume = {302.}, 
  number = {}, 
  pages = {}, 
  year = {2016}, 
  journal = {Advances in Intelligent Systems and Computing}
}

@article{LSD,
  author = {Brian Ichter, James Harrison, Marco Pavone} , 
  title = {Learning Sampling Distributions for Robot Motion Planning}, 
  volume = {}, 
  number = {}, 
  pages = {}, 
  year = {2017}, 
  journal = {International Conference on Robotics and Automation}
}

@article{OB,
  author = { Rodriguez, S. ; Xinyu Tang ; Jyh-Ming Lien ; N.M. Amato.} , 
  title = {An obstacle-based rapidly-exploring random tree}, 
  volume = {10.}, 
  number = {}, 
  pages = {1109}, 
  year = {2006}, 
  journal = {IEEE International Conference on Robotics and Automation}
}

@article{EEB,
  author = {Zhang, L., Manocha, D.:} , 
  title = {An efficient retraction-based RRT planner}, 
  volume = {302.}, 
  number = {}, 
  pages = {}, 
  year = {2008}, 
  journal = {Robotics and Automation, 2008. ICRA 2008. IEEE International Conference on, IEEE }
}

@article{ATD,
  author = {Jaillet, L., Yershova, A., La Valle, S.M., Siméon, T.} , 
  title = {Adaptive tuning of the sampling domain for dynamic-domain rrts}, 
  volume = {302.}, 
  number = {}, 
  pages = {2851–2856}, 
  year = {2005}, 
  journal = {Intelligent Robots and Systems}
}

@article{AOP,
  author = {Perez, A., Karaman, S., Shkolnik, A., Frazzoli, E., Teller, S., Walter, M.R.} , 
  title = {Asymptotically-optimal path planning for manipulation using incremental sampling-based algorithms}, 
  volume = {302.}, 
  number = {}, 
  pages = {4307–4313}, 
  year = {2011}, 
  journal = {IEEE/RSJ Int’l Conf. on Intelligent Robots and Systems (IROS)}
}

@article{Smart,
  author = {Islam, Fahad; Nasir, Jauwairia; Malik, Usman; Ayaz, Yasar; Hasan, Osman},
  title = {RRT*-Smart: Rapid convergence implementation of RRT* towards optimal solution}, 
  volume = {}, 
  number = {}, 
  pages = { 1651–1656}, 
  year = {2012}, 
  journal = {Proceedings of IEEE International Conference on Mechatronics and Automation }
}


@article{Informed,
  author = {Gammell, Jonathan D., Srinivasa, Siddhartha S., Barfoot, Timothy D.},
  title = {Informed RRT*: Optimal Sampling-based Path Planning Focused via Direct Sampling of an Admissible Ellipsoidal Heuristic}, 
  volume = {}, 
  number = {}, 
  pages = {2997-3004}, 
  year = {2014}, 
  journal = { IEEE/RSJ International Conference on Intelligent Robots and Systems }
}

@article{hRRT,
  author = {C. Urmson and R. Simmons},
  title = {Approaches for heuristically biasing
RRT growth}, 
  volume = {2}, 
  number = {}, 
  pages = {1178–1183}, 
  year = {2003}, 
  journal = { IROS }
}

@article{fbias,
  author = {S. Kiesel, E. Burns, and W. Ruml},
  title = {Abstraction-guided sampling for
motion planning}, 
  volume = {}, 
  number = {}, 
  pages = {}, 
  year = {2012}, 
  journal = {SoCS }
}

@article{RRM,
  author = {R. Alterovitz, S. Patil, and A. Derbakova},
  title = {Rapidly-exploring roadmaps:
Weighing exploration vs. refinement in optimal motion planning}, 
  volume = {}, 
  number = {}, 
  pages = {3706–3712}, 
  year = {2011}, 
  journal = {ICRA }
}

@article{RRT,
  author = {Steven M. Lavalle},
  title = {Rapidly-Exploring Random Trees: A New Tool for Path Planning}, 
  volume = {}, 
  number = {}, 
  pages = {}, 
  year = {1998}, 
  journal = {}
}

@article{PRM,
  author = {L. E. {Kavraki} and P. {Svestka} and J. {Latombe} and M. H. {Overmars}
},
  title = {Probabilistic roadmaps for path planning in high-dimensional configuration spaces}, 
  volume = {12}, 
  number = {4}, 
  pages = {566-580}, 
  year = {1996}, 
  journal = {IEEE Transactions on Robotics and Automation}
}

@article{EST,
  author = {D. Hsu, J. C. Latombe, and R. Motwani},
  title = {Path planning in expansive configuration spaces.}, 
  volume = {9}, 
  number = {4-5}, 
  pages = {495–512}, 
  year = {1999}, 
  journal = {International Journal of Computational Geometry and Applications}
}

@article{smooth,
  author = {Hauser, Kris and Ng-Thow-Hing, Victor},
  title = {Fast smoothing of manipulator trajectories using optimal bounded-acceleration shortcuts.}, 
  volume = {}, 
  number = {}, 
  pages = {2493 - 2498}, 
  year = {2010}, 
  journal = {IEEE International Conference on Robotics and Automation}
}

@article{oBIT,
  author = {Meng Z , Qin H , Sun H , et al},
  title = { Obstacle-guided informed planning towards robot navigation in cluttered environments}, 
  volume = {}, 
  number = {}, 
  pages = {}, 
  year = {2018}, 
  journal = {IEEE International Conference on Robotics & Biomimetics}
}

@article{BIT,
  author = {J. D. {Gammell} and S. S. {Srinivasa} and T. D. {Barfoot}},
  title = { Batch Informed Trees (BIT*): Sampling-based optimal planning via the heuristically guided search of implicit random geometric graphs}, 
  volume = {}, 
  number = {}, 
  pages = {3067-3074}, 
  year = {2015}, 
  journal = {IEEE International Conference on Robotics and Automation (ICRA)}
}

@article{RABIT, 
author={S. Choudhury and J. D. Gammell and T. D. Barfoot and S. S. Srinivasa and S. Scherer}, 
title={Regionally accelerated batch informed trees (RABIT*): A framework to integrate local information into optimal path planning}, 
year={2016}, 
volume={}, 
number={}, 
pages={4207-4214}, 
journal ={IEEE International Conference on Robotics and Automation (ICRA)}}
